Optimal Control of Wave Energy Converters Using Epsilon-Trig Regularization Method

The wave energy converter (WEC) devices provide access to a renewable energy source. Developing control strategies to harvest maximum wave energy requires solving a constrained optimal control problem. It is shown that singular control arcs may constitute part (or the entire) of extremal trajectories. Characterizing the optimal control structure, especially with the possibility of many switches between regular and singular control arcs, is challenging due to lack of \textit{a priori} information about: 1) optimal sequence as well as number of the regular and singular control arcs, and 2) the corresponding optimal switch times (from a regular to a singular arc and vice versa). This investigation demonstrates the application of a recently developed construct, the Epsilon-Trig Regularization Method (ETRM), to the problem of maximizing energy harvesting for a point-absorber WEC model in the presence of control constraints. Utility of the ETRM for the WEC problem is demonstrated by comparing its high-quality results against those in the literature for a number of test cases.

==> Acknowledgment.tex <==
\section*{ACKNOWLEDGEMENT}
The second author would like to thank Ossama Abdelkhalik and Shangyan Zou at Iowa State University regarding their help on the wave excitation functions.

==> Nomenclature.tex <==
\section*{NOMENCLATURE}
\begin{tabbing}
XXXXXXXX \= \kill% this line sets tab stop
BVP \> Boundary value problem\\
EOM \> Equation of motion\\
GLCC \> Generalized Legendre Clebsch condition\\
MPBVP \> Multi-point boundary value problem\\
OCP  \> Optimal control problem\\
OCT  \> Optimal control theory\\
PMP \> Pontryagin's Minimum Principle\\
PTO \> Power take-off\\
TPBVP \> Two-point boundary-value problem\\
UTM \> Unified Trigonometrization Method\\
WEC \> Wave energy converter\\\\  

 $H$ \> Hamiltonian\\
 $J$ \> Cost functional\\
 $L$ \> Lagrangian (path cost)\\
 $N$ \> Tangency conditions\\
 \\
 $t$ \> Time, s\\
 $t\textsubscript{f}$ \> Final time, s\\
 $$\bm{u}$ \> Control vector\\
 $u_{\epsilon}$ \> Error control\\
 $u$\textsubscript{TRIG}\> Trigonometric control\\
 $\bm{x}$ \> State vector\\
 \\
 $\epsilon_1$ \> Error parameter for control constraint\\
 $\epsilon_2$ \> Error parameter for state constraint\\
 $\bm{\lambda}$ \> Costate vector\\
 \textbf{$\Phi$} \> Terminal constraints\\
 \textbf{$\Pi$} \> Tangency constraint multipliers\\
 $\Psi$ \> Initial constraints\\ \hspace{0.1 in} 
\end{tabbing}


==> Preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{PRELIMINARIES} 
\label{sec:prelim}
\subsection{Formulation of Optimal Control Problem}
Let $\boldsymbol{x} \in \mathbb{R}^n$ and $\bm{u} \in \mathbb{R}^m$ denote the state and control vectors, respectively. The cost functional, $J$, for a standard OCP can be written in Bolza form as 
\begin{equation} 
J = \phi(\boldsymbol{x}(t_f),t_f,\boldsymbol{x}(t_0),t_0) + \int_{t_0}^{t_f} L(\boldsymbol{x}(t),\boldsymbol{u}(t),t)dt,
\end{equation}
where $\phi$ is the scalar terminal cost, $L$ is the running cost, $t_0$ and $t_f$ denote the initial and final limits of time, respectively. The cost functional is subject to a number of constraints usually written as
\begin{align}
\text{Differential equations:}& ~ \dot{\boldsymbol{x}}(t) = \boldsymbol{f}(\boldsymbol{x}(t),\boldsymbol{u}(t),t), \label{eq:EOM}\\
\text{Boundary constraints:}& ~\bm{\Psi}(\boldsymbol{x}(t_f),t_f,\boldsymbol{x}(t_0),t_0) = \textbf{0}, \\
%\text{Terminal constraints:}& ~\bm{\Phi}(\boldsymbol{x}(t_f),t_f) = \textbf{0}, \label{eq:TCs}  \\
\text{State path constraints:} &~\boldsymbol{x}\textsubscript{MIN} \leq \boldsymbol{x}(t) \leq \boldsymbol{x}\textsubscript{MAX,} \\
\text{Control constraints:} &~\boldsymbol{u}\textsubscript{MIN} \leq \boldsymbol{u}(t) \leq \boldsymbol{u}\textsubscript{MAX,}
\end{align}
where $\boldsymbol{x}$\textsubscript{MIN}, $\boldsymbol{x}$\textsubscript{MAX}, $\boldsymbol{u}$\textsubscript{MIN}, and $\boldsymbol{u}$\textsubscript{MAX} denote the specified lower and upper bounds for the states and controls, respectively. Also, $\bm{\Psi}$ $\in$ $\mathbb{R}^p$ for $p < n$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Necessary Conditions of Optimality using Calculus of Variations}  
A brief review of first-order necessary conditions of optimality is given since it allows us to elaborate on the details of the new construct and we are able to clarify different elements of the problem formulation in the remainder of the paper. A mathematical quantity called the Hamiltonian simplifies the derivation of the necessary conditions of optimality and is defined as \begin{equation}
\label{eqn:hamiltonian}
H = L(\boldsymbol{x},\boldsymbol{u},t) + \boldsymbol{\lambda}^T \boldsymbol{f}(\boldsymbol{x},\boldsymbol{u},t),
\end{equation}
where $\bm{\lambda} \in \mathbb{R}^n$ is the costate vector associated with the state vector. Costates have their corresponding dynamics, which is obtained through Euler-Lagrange equations.
\begin{equation}
\label{eqn:lambdadot}
\dot{\bm{\lambda}} = - \left [\frac{\partial H}{\partial \bm{x}} \right ]^T.
\end{equation}
Let $\Phi = \phi + \bm{\nu}^T \bm{\Psi}$ where $\bm{\nu} \in \mathbb{R}^p$ denote the vector of constant Lagrange multipliers, which are used to adjoin the boundary conditions to the cost functional. 
Eq.~\eqref{eqn:controllaw} shows the optimal control law, $\bm{u}(t)$, as a function of the states and costates, which is also known as the strong form of optimal control. Eqs.~\eqref{eqn:initialcond} and \eqref{eqn:terminalcond} specify the initial and terminal boundary conditions on the costates. It is possible for the final time, $t_f$ to be a parameter that has to be optimized. The free final time condition, shown by Eqs.~\eqref{eqn:timecond} and \eqref{eqn:timecond_0}, define conditions that have to be taken into account for free-final-time problems. Eqs. (\ref{eqn:lambdadot})--(\ref{eqn:timecond_0}) define the necessary conditions of optimality, and they form a well-defined TPBVP. BVP solvers such as MATLAB's bvp4c can solve such TPBVP. 
 \begin{equation}
\label{eqn:controllaw}
\frac{\partial H}{\partial \bm{u}} = 0,
\end{equation}
\begin{equation}
\label{eqn:initialcond}
\bm{\lambda}(t_0)^T + \frac{\partial \Phi}{\partial \bm{x}(t_0)} = \textbf{0}, 
\end{equation}
\begin{equation}
\label{eqn:terminalcond}
\bm{\lambda}(t_f)^T - \frac{\partial \Phi}{\partial \bm{x}(t_f)} = \textbf{0},
\end{equation}
\begin{equation}
\label{eqn:timecond}
\left(H + \frac{\partial \Phi}{\partial t} \right)_{t=t_f} = 0. 
\end{equation}
\begin{equation} \label{eqn:timecond_0}
\left(H - \frac{\partial \Phi}{\partial t} \right)_{t=t_0} = 0. 
\end{equation}
When more than one option exists after solving Eq.~\eqref{eqn:controllaw}, Pontryagin's minimum principle (PMP) helps select the optimal control as shown in Eq.~\eqref{eqn:pontryagin}, where superscript `*' refers to the optimal value \cite{longuski2014optimal}. It states that the optimal control will minimize the Hamiltonian, $H$, for all admissible values of control \cite{longuski2014optimal}.
\begin{equation}
\label{eqn:pontryagin}
H(t,\bm{x}^{*}(t),\bm{u^{*}}(t),\bm{\lambda^{*}}(t)) \leq H(t,\bm{x}^{*}(t),\bm{u}(t),\bm{\lambda^{*}}(t)).
\end{equation}
For all OCPs in this paper, it is assumed that $t_0 = 0$ seconds and is fixed. In addition, the final time $t_f$ is also fixed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bang-Bang Control and Singular Arcs}  
\label{sec:bangbang}
Suppose a bounded OCP with a scalar control, $u$, has a Hamiltonian, $H$, as shown in Eq.~\eqref{eqn:bangbangHam}.\cite{longuski2014optimal} The control is allowed to take values between its admissible lower and upper limits denoted by $-u\textsubscript{LIM}$ and $u\textsubscript{LIM}$, respectively. Since $H$ is linear in $u$, Eq.~\eqref{eqn:controllaw} results in Eq.~\eqref{eqn:switchingfcn}.
\begin{equation}
\label{eqn:bangbangHam}
H = H_{0}(t,\bm{x}(t),\bm{\lambda}(t)) + H_{1}(t,\bm{x}(t),\bm{\lambda}(t))u,
\end{equation}
\begin{equation}
\label{eqn:switchingfcn}
\frac{\partial H}{\partial{u}} = H_{1}. 
\end{equation}
The choice of $u$ cannot influence $H_{0}(t,\bm{x}^{*}(t),\bm{\lambda}(t))$, so the solution process ignores this term. If $H_{1}$ is positive, then the solution process should take the lowest value of $u$ to minimize $H$. Similarly, if $H_{1}$ is less than 0 units, the process should take the maximum value of $u$. In summary, the PMP gives the control law shown in Eq.~\eqref{eqn:summarybang}.
\begin{equation}
\label{eqn:summarybang}
u = 
\begin{cases}
-u\textsubscript{LIM}, & \text{if } H_{1}  > 0,\\
\in [-u\textsubscript{LIM},u\textsubscript{LIM}], & \text{if } H_{1} = 0,\\
u\textsubscript{LIM}, & \text{if } H_{1} < 0.\\
\end{cases}
\end{equation}
OCT defines the coefficient $H_{1}(t,\bm{x}^{*}(t),\bm{\lambda}(t))$ as the switching function. When $H_{1}$ alternates between positive and negative values, the control law switches back and forth between its lower and upper bounds, attaining a profile known as ``bang-bang". When $H_{1}\equiv 0$ during one (or multiple) non-zero time interval(s), say $t_{0} \leq t_{1} <t_{2} \leq t_f$, then the subarc [$t_{1}$,$t_{2}$] becomes a singular subarc and the control no longer influences $H$, leading to non-uniqueness issues. To determine unique candidate singular controls, the traditional approach differentiates Eq.~\eqref{eqn:controllaw} with respect to time as shown in Eq.~\eqref{eqn:singularcontrol}. The last term in Eq.~\eqref{eqn:singularcontrol} vanishes because the derivative of Hamiltonian with respect to the control, ${H_{u}}$, does not contain $u$ and $\frac{\partial{H_{u}}}{\partial{u}}$ becomes 0 as a result.
\begin{equation}
\label{eqn:singularcontrol}
\dot{H}_{u} = 0 = \frac{\partial{H_{u}}}{\partial{t}} + \left [ \frac{\partial{H_{u}}}{\partial{\bm{x}}} \right ]^T \dot{\bm{x}} + \left [ \frac{\partial{H_{u}}}{\partial{\bm{\lambda}}} \right ]^T \dot{\bm{\lambda}} + \left [ \frac{\partial{H_{u}}}{\partial{\bm{u}}} \right ]^T \dot{\bm{u}}.
\end{equation}
The solution process forms $\frac{d^{2}}{dt^{2}}H_{u}$ $\equiv$ 0, and if $u$ appears explicitly, the process uses the condition specified in Eq.~\eqref{eqn:singularcontrol} along with the Generalized Legendre-Clebsch Condition (GLCC) as shown in Eq.~\eqref{eqn:kelley} to determine the singular control law. If $u$ does not appear explicitly, the solution process takes even time derivatives of $H_{u}$ until the process satisfies GLCC along with the conditions specified by odd time-derivatives of $H_{u}$ \cite{longuski2014optimal} to obtain the singular control law.

\begin{equation}
\label{eqn:kelley}
(-1)^{q}\frac{\partial}{\partial{u}}\left(\frac{d^{2q}H^{*}_{u}}{{dt^{2q}}}\right) \geq 0.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Path Constraints}
\label{sec:path}
The presence of path constraints further complicates the formulation of OCP by introducing corner conditions in certain costates and effectively splitting the trajectory into multiple arcs. Path constraints are usually of the form shown in Eq.~\eqref{eqn:pathconstraint}. To obtain the control history for the constrained arc, the solution process takes time derivatives of the path constraints until a control variable appears explicitly. If this happens with the $q^{\text{th}}$ derivative, the solution process augments the Hamiltonian as shown in Eq.~\eqref{eqn:hamiltonian_path}, and obtains the control law for the constraint boundary by solving $\bm{S}^{(q)} = 0$. \cite{longuski2014optimal,bryson:path1963} 
\begin{equation}
\label{eqn:pathconstraint}
\bm{S}(\bm{x},t) \leq 0,
\end{equation}
\begin{equation}
\label{eqn:hamiltonian_path}
H = L + \bm{\lambda}^T \bm{f} + \bm{\mu}^T\bm{S}^{q}.
\end{equation}

The addition of path constraints also modifies the dynamic equations of the costates along the constrained arcs as shown in Eq.~\eqref{eqn:lambdadot2}, where Eq.~\eqref{eqn:mueqn} determines the multipliers $\bm{\mu}$.
\begin{equation}
\label{eqn:lambdadot2}
\dot{\bm{\lambda}} = - \left [\frac{\partial H}{\partial \bm{x}} \right ]^T = -L_{\bm{x}} - \bm{\lambda}^T \bm{f}_{\bm{x}} - \bm{\mu}^T \bm{S_x}^{q},
\end{equation}
\begin{equation}
\label{eqn:mueqn}
\frac{\partial H}{\partial \bm{u}} = L_{\bm{u}} + \bm{\lambda}^T \bm{f_u} + \bm{\mu}^T \bm{S_u}^{q} = 0.
\end{equation}

The states are continuous at the entry ($t_1$) and exit ($t_2$) of the constrained arc as shown in Eq.~\eqref{eqn:statecontinuity}. The solution process chooses corner conditions on costates such that the costates are continuous at the exit of the constrained arc as shown in Eq.~\eqref{eqn:exitconditions}. The tangency conditions described in Eq.~\eqref{eqn:tangencycond} and corner conditions in Eq.~\eqref{eqn:costatecornercond} and Eq.~\eqref{eqn:hamcornercond} apply at the entry point of the constrained arc, where $\bm{\Pi}$ are the multipliers corresponding to the tangency constraint conditions. $\bm{N}_x$ and $\bm{N}_t$ are the derivatives of tangency constraints, $\textbf{N}$ as shown in Eq.~\eqref{eqn:costatecornercond} and Eq.~\eqref{eqn:hamcornercond}, respectively.
\begin{equation}
  \begin{aligned}
    \bm{x}({t_1}^{+}) =&\ \bm{x}({t_1}^{-}),\\
    \bm{x}({t_2}^{+}) =&\ \bm{x}({t_2}^{-}),
    \label{eqn:statecontinuity}
  \end{aligned}
\end{equation}
\begin{equation}
  \begin{aligned}
    \bm{\lambda}({t_2}^{+}) =&\ \bm{\lambda}({t_2}^{-}),\\
    H({t_2}^{+}) =&\ H({t_2}^{-}),
    \end{aligned}
    \label{eqn:exitconditions}
\end{equation}
\begin{equation}
\label{eqn:tangencycond}
\bm{N}(\bm{x},t) =\begin{bmatrix}S(\bm{x},t),S^{1}(\bm{x},t),...,S^{q-1}(\bm{x},t)\end{bmatrix}^{T},
\end{equation}
\begin{equation}
\label{eqn:costatecornercond}
\bm{\lambda}({t_1}^{+}) = \bm{\lambda}({t_1}^{-}) + \bm{\Pi}^T \bm{N}_{\bm{x}},
\end{equation}
\begin{equation}
\label{eqn:hamcornercond}
H({t_1}^{+}) = H({t_1}^{-})  + \bm{\Pi}^T \bm{N}_t.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Additional Necessary Conditions} 
\label{sec:addcond}
While the relations in Section \ref{sec:path} are known to most of the researchers, there are additional conditions that have to considered. Eq.~\eqref{eqn:add_nec_cond} states the additional necessary conditions needed for OCPs with path constraints in a general form, where $q$ is the order of the path constraint. \cite{bryson:path1963,jacobson:path1971,kreindler:path1982} Note that the superscript for $\mu$ represent the order of its time-derivative.
\begin{subequations}
\label{eqn:add_nec_cond}
\begin{align}
\Pi_{k-1} - (-1)^{q-k}\mu^{q-k}(t_{\rm{1}}^{+}) & 
\begin{cases}
\geq 0,\quad\rm{if}\quad k = 1,\\
= 0,\quad\rm{if}\quad k = 2,...,q; q >1,\\
\end{cases}\label{eqn:add_nec_cond1}\\
(-1)^{q-k}\mu^{q-k}(t_{\rm{2}}^{-}) & 
\begin{cases}
\geq 0,\quad\rm{if}\quad k = 1,\\
= 0,\quad\rm{if}\quad k = 2,...,q; q >1,\\
\end{cases}\label{eqn:add_nec_cond2}\\
(-1)^{q}\mu^{q}(t) &\geq 0,\quad\rm{if}\quad t \in [t_{\rm{1}},t_{\rm{2}}].\label{eqn:add_nec_cond3}
\end{align}
\end{subequations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Epsilon-Trig Regularization Method for Bang-Bang and Singular Control Problems}
Silva and Tr\'elat \cite{silva2010smooth} developed a smooth regularization method to alleviate some of the issues associated with non-smoothness of the control that affects the solution procedure of the resulting BVPs when indirect optimization methods are used. Recently, Mall and Grant developed a new regularization method that presents distinct features by not only smoothing the control input, but also by resolving the dimensional inconsistency that can occur in Ref. \cite{silva2010smooth}. This new method, called as the Epsilon-Trig regularization method, utilizes an error parameter, $\epsilon$, while the controls are posed in a trigonometric form \cite{mall2017epsilon}. Application of the Epsilon-Trig method is demonstrated on a number of challenging problems including a scramjet based impactor \cite{williams2017trajectory}. For certain types of problems, application of the strong form of optimality, i.e., $\partial H/\partial u = 0$ (see Eq.~\eqref{eqn:controllaw}), may lead to a transcendental form, which often prevents the construction of a closed-form solution for control \cite{mall2016trigonomerization}. It is shown that the Epsilon-Trig method in conjunction with the introduction of another differential equation can overcome the issue associated with transcendental form, and instead, results in a closed-form expression \cite{mall2016trigonomerization}.

The most prominent feature of the Epsilon-Trig method is its ability to capture both regular and singular control arcs using a simple and innovative regularization. The OCP can be reformulated to have only one control, $u$\textsubscript{TRIG}, instead of having multiple controls as suggested in the smooth regularization method. Trigonometric functions can then be used upon the control to form two orthogonal components, one is the smoothed control and the other is the error control. As shown in Fig.~\ref{fig:epsilontrig}, the control can attain a maximum value of $u\textsubscript{LIM}$ units for OB, for the original normalized bang-bang control problem indicated in red. The smoothed bang-bang control is represented by OA indicated in green, and the error control is represented by BA.
\begin{figure}[!htb]
\centering
\includegraphics[width = 3.2in]{epsilontrig}
\caption{Smoothing of control using Trigonometrization.}
\label{fig:epsilontrig}
\end{figure}

It should be noted that the smoothed control, $u\textsubscript{LIM} \sin(u\textsubscript{TRIG})$, and the error control, $u\textsubscript{LIM} \cos(u\textsubscript{TRIG})$, are present only in one state equation respectively as shown in Eq.~\eqref{eqn:epsilontrig}. This makes the entire system very simple to solve and ensures that the new system of equations is very close to the original system. 
\begin{subequations}
\label{eqn:epsilontrig}
\begin{align}
\text{Minimize: } J &= J(t_{f},\boldsymbol{x}(t_{f})),\label{eqn:epsilontrig1}\\
\text{Subject to: }\dot{x}_{\epsilon} &= f_{1}(t,\boldsymbol{x}) + \epsilon u_{\text{LIM}}\cos u\textsubscript{TRIG},\label{eqn:epsilontrig2}\\
\dot{x}_{n} &= f_{n}(t,\boldsymbol{x}),\label{eqn:epsilontrig3}\\
\dot{x}_{k+1} &= f_{k+1}(t,\boldsymbol{x}) + u_{\text{LIM}}\sin u\textsubscript{TRIG}.\label{eqn:epsilontrig4}
\end{align}
\end{subequations}

Using Eq.~\eqref{eqn:controllaw}, the optimal control options are shown in Eq.~\eqref{eqn:trigcontrol}. The smoothed control, sin $u$\textsubscript{TRIG}, and the error control, cos $u$\textsubscript{TRIG}, can then be computed. 
\begin{equation}
\label{eqn:trigcontrol}
u\textsubscript{TRIG}^{*} = 
\begin{cases}
\arctan \left(\dfrac{\lambda_{x\textsubscript{k+1}}}{\epsilon\lambda_{x\textsubscript{1}}}\right),\\\\
\arctan \left(\dfrac{\lambda_{x\textsubscript{k+1}}}{\epsilon\lambda_{x\textsubscript{1}}}\right) + \pi.
\end{cases}
\end{equation}

In Ref. \cite{mall2017epsilon} it is shown that the Epsilon-Trig method is able to solve bounded control OCPs with realistic error controls. Moreover, the error parameter, $\epsilon$, becomes dimensionally consistent since it is present in only one state equation. A recently developed approach used in the OCT to impose state constraints upon the OCPs is discussed as follows. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Trigonometrization of Optimal Control Problems with State Constraints}
In order to impose bounds on the states of the OCP, the path cost, $L$, needs to be modified to $\tilde{L}$ as shown in Eq.~\eqref{eqn:newL}. In this equation, $i$ ranges from 1 to $n$, where $n$ is the number of states with pure state constraints.

\begin{equation}
\label{eqn:newL}
\tilde{L} = L + \sum_{i=1}^{n} \epsilon_{i}\sec\left(\dfrac{\pi}{2}\left(\dfrac{2x_{i} - x_{i\textsubscript{MAX}} - x_{i\textsubscript{MIN}}}{x_{i\textsubscript{MAX}} - x_{i\textsubscript{MIN}}}\right)\right).
\end{equation}

Eq.~\eqref{eqn:newLsimpler} is a simpler reformulation of Eq.~\eqref{eqn:newL}, where $x_{i\textsubscript{MIN}}$ and $x_{i\textsubscript{MAX}}$ have the same magnitude. Furthermore, Eq.~\eqref{eqn:newLsimpler} can be used for one sided state constraints, where $x_{i\textsubscript{LIM}}$ is the upper or the lower limit on the state $x_{i}$. Note that if $x_{i\textsubscript{LIM}}$ is 0, Eq.~\eqref{eqn:newL} should be used along with a reasonably large magnitude for the opposite limit of $x_{i}$.
\begin{equation}
\label{eqn:newLsimpler}
\tilde{L} = L + \sum_{i=1}^{n}\epsilon_{i}\sec\left(\dfrac{\pi}{2}\left(\dfrac{x_{i}}{x_{i\textsubscript{LIM}}}\right)\right).
\end{equation}

The main idea in Eqs.~\eqref{eqn:newL} and \eqref{eqn:newLsimpler} is to bound states by introducing trigonometric regularization functions such that the new path cost, $\tilde{L}$, gains an infinite value when the path constraint becomes active. Since the objective is also to reduce $\tilde{L}$, the solver avoids gaining infinite values for the objective functional. Moreover, the problem involves continuous derivatives of the states and costates. Therefore, $H$ and $\tilde{L}$ cannot have infinite values and the BVP solver, \textit{bvp4c}, avoids large values of $\tilde{L}$. Additionally, the trigonometric regularization functions affect the costate equations. Since the controls depends on the costates, $\tilde{L}$ impact the controls and eventually the states. Thus, the bounds on the states are imposed indirectly and very simply using the trigonometric regularization functions of secant form. Ref. \cite{wang2017indirect} suggests the use of a quadratic $\tan$ function. It was found that using a linear trigonometric function, $\sec$, results in more accurate solutions and a simpler problem formulation. Therefore, this study uses Eq.~\eqref{eqn:newLsimpler} to impose state constraints for the considered WEC problem. The regularization approach that combines and improves upon the ideas presented in the Epsilon-Trig method and Trigonometrization of OCPs with state constraints is presented in the next subsection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background of the Unified Trigonometrization Method} 
Instead of solving a complicated MPBVP with its associated difficulties discussed in Sections \ref{sec:path} and \ref{sec:addcond}, an approach based on trigonometric regularization of the OCP, dubbed the Unified Trigonometrization Method (UTM), was used to solve a simpler TPBVP. As the name suggests, the UTM unifies and improves upon different methods that employ trigonometry to bound the states and controls of the OCPs. Consider an OCP with the following characteristics and assumptions: 
\begin{enumerate}
\item The OCP contains $l$ (for $l = 0, \cdots, i$) controls that appear in a linear form in the Hamiltonian as shown in Eq.~\eqref{eqn:HamType1}, where $H_{1_{i}}$ is the switching function associated with the $i$-th control input, $u_i$. 
\item There are $m$ bounded controls that appear in the Hamiltonian of the OCP in a nonlinear form, $f_{j}(u_{j}(t))$, as shown in Eq.~\eqref{eqn:HamType2}. 
\item The control constraints are of the form $u_{i,j\textsubscript{MIN}} \leq u_{i,j} \leq u_{i,j\textsubscript{MAX}}$, where $i$ ranges from 0 to $l$ and $j$ ranges from 0 to $m$.
\item The OCP contains $n$ along-the-path state constraints of the form $S_{k\textsubscript{MIN}} \leq S_{k} \leq S_{k\textsubscript{MAX}}$, where $k$ ranges from 0 to $n$.
\item For simplicity of discussion, each control appears in only one state equation of motion (EOM).
\item There are $a$ state EOMs without any control constraints and $i + j$ state EOMs with control constraints. 
\end{enumerate}

\begin{subequations}
\label{eqn:HamTypes}
\begin{align}
H_{i} &= H_{0_{i}}(t,\boldsymbol{x},\bm{\lambda}) + H_{1_{i}}(t,\boldsymbol{x},\bm{\lambda})u_{i},\label{eqn:HamType1}\\
H_{j} &= H_{0_{j}}(t,\boldsymbol{x},\bm{\lambda}) + H_{1_{j}}(t,\boldsymbol{x},\bm{\lambda})f_{j}(u_{j}).\label{eqn:HamType2}
\end{align}
\end{subequations}

This OCP can be regularized by introducing trigonometric regularization parameters (minuscule errors) into the path cost, $L$, to obtain a new path cost, $\tilde{L}$, and modifying the cost functional $J$ to the form shown in Eq.~\eqref{eqn:utmbbs1}. $\tilde{L}$, as shown in Eq.~\eqref{eqn:utmbbs2}, consists of the terms $\epsilon_{i}\cos{u_{i\textsubscript{TRIG}}}$, which account for regularizing $l$ bang-bang and singular controls. $\tilde{L}$ also contains the terms $\epsilon_{k}$sec terms to impose the $n$ state constraints, $S_{k}$, upon the OCP. The state EOMs without any control constraints are kept unmodified as shown in Eq.~\eqref{eqn:utmbbs3}. The state EOMs shown in Eq.~\eqref{eqn:utmbbs4} contain bounded controls, $u_{i,j}$. In Eq.~\eqref{eqn:utmbbs}, $f_{a}$ is dependent on the time, states, and unconstrained controls, $\boldsymbol{u}\textsubscript{UC}$; $f_{i}$, $f_{j}$, and $g_{i}$ are dependent only on the time and states; and $g_{j}$ is dependent on the time, states, and bounded controls, $u_{j}$. 
\begin{subequations}
\label{eqn:utmbbs}
\begin{align}
J &= \phi(\boldsymbol{x}(t_f),t_f,\boldsymbol{x}(t_0),t_0) + \int_{t_0}^{t_f} \tilde{L}(\boldsymbol{x},\boldsymbol{u},t)\mathrm{d}t,\label{eqn:utmbbs1}\\
\tilde{L} &= L + \sum_{i=1}^{l}\epsilon_{i}\cos{u_{i\textsubscript{TRIG}}}\notag\\
&\ + \sum_{k=1}^{n}\epsilon_{k}\sec\left(\dfrac{\pi}{2}\left(\dfrac{2S_{k} - S_{k\textsubscript{MAX}} - S_{k\textsubscript{MIN}}}{S_{k\textsubscript{MAX}} - S_{k\textsubscript{MIN}}}\right)\right),\label{eqn:utmbbs2}\\
\dot{x}_{a} &= f_{a}(t,\boldsymbol{x},\boldsymbol{u\textsubscript{UC}}),\label{eqn:utmbbs3}\\
\dot{x}_{i} &= f_{i}(t,\boldsymbol{x}) + g_{i}(t,\boldsymbol{x})u_{i},\label{eqn:utmbbs4}\\
\dot{x}_{j} &= f_{j}(t,\boldsymbol{x}) + g_{j}(t,\boldsymbol{x},u_{j}).\label{eqn:utmbbs5}
\end{align}
\end{subequations}

The bounded controls are converted to a trigonometric form as shown in Eq.~\eqref{eqn:utmcontrol1}. The expressions used for $c_{0_{i,j}}$ and $c_{1_{i,j}}$ in Eq.~\eqref{eqn:utmcontrol1} are shown in Eq.~\eqref{eqn:utmcontrol2} and Eq.~\eqref{eqn:utmcontrol3}, respectively. 
\begin{subequations}
\label{eqn:utmcontrol}
\begin{align}
u_{i,j} &= c_{1_{i,j}}\sin u_{i,j\textsubscript{TRIG}} + c_{0_{i,j}},\label{eqn:utmcontrol1}\\
c_{0_{i,j}} &= \dfrac{u_{i,j\textsubscript{MAX}} + u_{i,j\textsubscript{MIN}}}{2},\label{eqn:utmcontrol2}\\
c_{1_{i,j}} &= \dfrac{u_{i,j\textsubscript{MAX}} - u_{i,j\textsubscript{MIN}}}{2}.\label{eqn:utmcontrol3}
\end{align}
\end{subequations}
Using Eq.~\eqref{eqn:controllaw}, the optimal control options for the $l$ bang-bang and singular controls are shown in Eq.~\eqref{eqn:utmbbscontrol}, where $H_{1_{i}}$ are the switching functions for the respective controls. Similarly, the optimal control options are generated for the other $m$ bounded controls using Eq.~\eqref{eqn:controllaw} and are shown in Eq.~\eqref{eqn:trigctrl}. The values $\pm\pi$/2 for $u_{j\textsubscript{TRIG}}$ restrict control, $u_{j}$, between $u_{j\textsubscript{MIN}}$ and $u_{j\textsubscript{MAX}}$. The unbounded values for $u_{j}$ are expected when $u_{j\textsubscript{TRIG}}$ is $h_{j}(t,x,\lambda)$, which includes a complicated $\arcsin$ term. It may happen that the value inside the $\arcsin$ term becomes less than -1 or more than 1, leading to imaginary values for this term. In such cases, the control, $u_{j}$, is evaluated based on PMP with only two options for $u_{j\textsubscript{TRIG}}$, $\pm\pi$/2.
\begin{equation}
\label{eqn:utmbbscontrol}
u_{i\textsubscript{TRIG}}^{*} = 
\begin{cases}
\arctan\left(\dfrac{c_{1_{i}}H_{1_{i}}}{\epsilon_{i}}\right),\\\\
\arctan\left(\dfrac{c_{1_{i}}H_{1_{i}}}{\epsilon_{i}}\right) + \pi,
\end{cases}
\end{equation}

\begin{equation}
\label{eqn:trigctrl}
u_{j\textsubscript{TRIG}}^{*} = 
\begin{cases}
\dfrac{-\pi}{2},\\
h_{j}(t,x,\lambda),\\
\dfrac{\pi}{2}.
\end{cases}
\end{equation}

Thus, the complicated OCP with bang-bang and singular controls, bounded controls, mixed state-control constraints, and pure state constraints can be solved using the UTM. The UTM improves upon the Epsilon-Trig method by including the error parameter and the error control in the path cost, $L$. Thus, the control options become independent of the costates and numerical issues are prevented when these costates vanish. Additionally, the UTM can solve other types of OCPs with control constraints and non-linear controls in their Hamiltonian as specified in \cite{mall2016trigonomerization,udani2017optimal}. The most salient features of the UTM are summarized as follows.
\begin{enumerate}
\item The singular control law is calculated without using the complicated traditional approach involving the Generalized Legendre Clebsch condition in conjunction with taking higher-order time derivatives of the switching function..
\item A simpler TPBVP is solved instead of a complicated MPBVP.
\item The bounds on the controls and states are placed in an automated and implicit manner at multiple places throughout the solution structure.
\item Additional necessary conditions, Lagrange multipliers and jump conditions corresponding to the control and path constraints are not required.   
\end{enumerate}
The idea used in the UTM to resolve issues with the bang-bang and singular control problems is an improvement upon the Epsilon-Trig method. The next section details the mathematical problem statement and its solution using the UTM.   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> futurework.tex <==
\section{FUTURE WORK}
In this study, a generic one degree-of-freedom point-absorber WEC is considered and the energy is harvested only through the heave motion of buoy. More energy can be harvested using a nonlinear model of the WEC \cite{richter2013nonlinear,abdelkhalik2018optimization}, which considers other motions including the surge of the wave as well. Moreover, the non-linear terms become effective as the velocity and amplitude forces increase \cite{ringwood2014control}. Future work thus involves demonstrating the utility of the ETRM for developing optimal control strategies pertaining point-absorber WECs with a three degree-of-freedom model and by taking into account non-linear contributing factors.
